Long-Term Employment Effects of the Minimum Wage in Germany: New Data and Estimators

We study the long-term effects of the 2015 German minimum wage introduction and its subsequent increases on regional employment. Using data from two waves of the Structure of Earnings Survey allows us to estimate models that account for changes in the minimum wage bite over time. While the introduction mainly affected the labour market in East Germany, the raises are also increasingly affecting low-wage regions in West Germany, such that around one third of regions have changed their (binary) treatment status over time. We apply different specifications and extensions of the classic difference-in-differences approach as well as a set of new estimators that enables for unbiased effect estimation with a staggered treatment adoption and heterogeneous treatment effects. Our results indicate a small negative effect on dependent employment of 0.5 percent, no significant effect on employment subject to social security contributions, and a significant negative effect of about 2.4 percent on marginal employment until the first quarter of 2022. The extended specifications suggest additional effects of the minimum wage increases, as well as stronger negative effects on total dependent and marginal employment for those regions that were strongly affected by the minimum wage in 2015 and 2019.

==> Tables/Incremental_1418_BIP.tex <==
% Table generated by Excel2LaTeX from sheet 'Incremental_1418_BIP'
\begin{table}[htbp]
  \centering
 \caption{Effects of the minimum wage introduction and its raises on regional employment \textbf{With ``GDP per capita x quarter'' as additional control}}
  \label{tab:incremental_VSE1418_allRaises_bip}
    \begin{tabular}{lccc}
    \toprule
    \toprule
    \multicolumn{1}{l}{} & (1)   & (2)  & (3) \\
    \multicolumn{1}{l}{VARIABLES} & Dependent  & Employment  & Marginal  \\
   & employment  & subject to SSC  & employment  \\
    \midrule
    \multicolumn{1}{l}{} &       &       &  \\
    \multicolumn{1}{l}{Treatment 2014   } & -0.00295** & -0.000136 & -0.0112* \\
    \multicolumn{1}{l}{} & (0.00144) & (0.00152) & (0.00589) \\
    \multicolumn{1}{l}{Placebo} & 0.000601 & 0.00142 & -0.00125 \\
    \multicolumn{1}{l}{} & (0.00111) & (0.00107) & (0.00245) \\
    \multicolumn{1}{l}{Treatment 2014 x (Time $>$ 2016)} & -0.00250 & 0.00151 & -0.0171*** \\
    \multicolumn{1}{l}{} & (0.00251) & (0.00256) & (0.00499) \\
    \multicolumn{1}{l}{Treatment 2018 x (Time $>$ 2018)} & -0.00773*** & -0.00627*** & -0.0181*** \\
    \multicolumn{1}{l}{} & (0.00236) & (0.00240) & (0.00545) \\
    \multicolumn{1}{l}{Treatment 2018 x (Time $>$ 2019)} & -0.000188 & 0.000870 & -0.00580*** \\
    \multicolumn{1}{l}{} & (0.00113) & (0.00115) & (0.00216) \\
    \multicolumn{1}{l}{Treatment 2018 x (Time $>$ 2020)} & 0.000748 & 0.000969 & -0.000631 \\
    \multicolumn{1}{l}{} & (0.000966) & (0.00102) & (0.00246) \\
    \multicolumn{1}{l}{Treatment 2018 x (Time $>$ 2021)} & -0.000849 & -0.000882 & -0.000636 \\
    \multicolumn{1}{l}{} & (0.000654) & (0.000688) & (0.00189) \\
    %\multicolumn{1}{l}{Constant} & 12.58*** & 12.06*** & 10.87*** \\
    %\multicolumn{1}{l}{} & (0.574) & (0.570) & (1.106) \\
    %\multicolumn{1}{l}{} &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Observations} & 9,509 & 9,509 & 9,509 \\
    \multicolumn{1}{l}{R$^{2}$ (within)} & 0.605 & 0.588 & 0.500 \\
    \midrule
    \multicolumn{1}{l}{Labour market region FE} & X     & X     & X \\
    \multicolumn{1}{l}{Quarter FE} & X     & X     & X \\
    \multicolumn{1}{l}{Controls} & X     & X     & X \\
    \bottomrule
    \bottomrule
    \end{tabular}%
\caption*{\scriptsize Source: Statistic of the Federal Employment Agency, SES 2014, 2018; own calculations. Note: The treatment effects refer to the coefficients $\beta$, $\delta_{2016}$, and $\delta_{\tau}$ in Equation (\ref{eq:equation3}). The binary treatment 2014 (2018) equals 1 if the regional wage gap in 2014 (2018) is equal to or above the population-weighted median. The control variables included are interactions of: time, east, and population share between 18 and 64 years in 2013; time, east, and type of labour market region; time, east, and employment share in different sectors; time and GDP per capita in 2013. Standard errors (in parentheses) are clustered at the level of the labour market regions. Confidence level: ***p$<$0.01, **p$<$0.05, *p$<$0.1.}
\end{table}%


==> Tables/Main_new.tex <==
\begin{table}[htbp]
  \centering
  \caption{Effects of the minimum wage introduction on regional employment}
  \label{tab:results_main_bip}
    \begin{tabular}{lccc}
    \toprule
    \toprule
    \multirow{2}{2cm}{VARIABLES} & Dependent & Employment  & Marginal  \\
    & employment & subject to SSC  & employment  \\
    \midrule
    \multicolumn{4}{l}{\textbf{Panel A: Binary treatment (wage gap)}} \\
    \multicolumn{1}{l}{Treatment} & -0.00511* & 0.000456 & -0.0239*** \\
    \multicolumn{1}{l}{} & (0.00260) & (0.00286) & (0.00763) \\
    \multicolumn{1}{l}{Placebo} & 0.000569 & 0.00142 & -0.00140 \\
    \multicolumn{1}{l}{} & (0.00111) & (0.00107) & (0.00246) \\
          &       &       &  \\
    \multicolumn{1}{l}{R$^{2}$ (within)} & 0.597 & 0.584 & 0.472 \\
          &       &       &  \\
     \multicolumn{4}{l}{\textbf{Panel B: Binary treatment (wage gap) interacted with growth}} \\
    \multicolumn{1}{l}{Treatment} & -0.00396 & 0.000415 & -0.0181** \\
    \multicolumn{1}{l}{} & (0.00339) & (0.00369) & (0.00887) \\
    \multicolumn{1}{l}{Placebo} & 0.00104 & 0.00195* & -0.000994 \\
          & (0.00108) & (0.00103) & (0.00243) \\
    \multicolumn{1}{l}{Treatment x Low growth 2010-2013} & -0.00698 & -0.00222 & -0.0267** \\
    \multicolumn{1}{l}{} & (0.00597) & (0.00694) & (0.0121) \\
          &       &       &  \\
    \multicolumn{1}{l}{R$^{2}$ (within)} & 0.605 & 0.590 & 0.484 \\
          &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Observations} & 9,509 & 9,509 & 9,509 \\
    \midrule
    \multicolumn{1}{l}{Labour Market Region FE} & X     & X     & X \\
    \multicolumn{1}{l}{Quarter FE} & X     & X     & X \\
    \multicolumn{1}{l}{Controls} & X     & X     & X \\
    \bottomrule
    \bottomrule
    \end{tabular}%
  \caption*{\scriptsize Source: Regional Statistic of the Federal Employment Agency; SES 2014; Federal Statistical Office; Federal Institute for Research on Building, Urban Affairs and Spatial Development; own calculations. Note: The treatment effect refers to the coefficient $\beta$ in Equation (\ref{eq:equation1}), estimated with TWFE. The binary treatment equals 1 if the regional wage gap is equal to or above the population-weighted median. 
  The control variables included are interactions of: time, east, and population share between 18 and 64 years in 2013; time, east, and type of labour market region; time, east, and employment share in different sectors; time and GDP per capita in 2013. The specification in Panel B additionally includes the interactions of time and the indicator for a low GDP between 2010 and 2013. Standard errors (in parentheses) are clustered at the level of the labour market regions. Confidence level: ***p$<$0.01, **p$<$0.05, *p$<$0.1.}
\end{table}%

